Shift Happens: Adjusting Classifiers

Minimizing expected loss measured by a proper scoring rule, such as Brier score or log-loss (cross-entropy), is a common objective while training a probabilistic classifier. If the data have experienced dataset shift where the class distributions change post-training, then often the model's performance will decrease, over-estimating the probabilities of some classes while under-estimating the others on average. We propose unbounded and bounded general adjustment (UGA and BGA) methods that transform all predictions to (re-)equalize the average prediction and the class distribution. These methods act differently depending on which proper scoring rule is to be minimized, and we have a theoretical guarantee of reducing loss on test data, if the exact class distribution is known. We also demonstrate experimentally that, when in practice the class distribution is known only approximately, there is often still a reduction in loss depending on the amount of shift and the precision to which the class distribution is known.

==> references.tex <==
@article{banerjee2005optimality,
  title={On the optimality of conditional expectation as a {Bregman} predictor},
  author={Banerjee, Arindam and Guo, Xin and Wang, Hui},
  journal={IEEE Trans. on Information Theory},
  volume={51},
  number={7},
  pages={2664--2669},
  year={2005},
  publisher={IEEE}
}

@article{merkle2013choosing,
  title={Choosing a strictly proper scoring rule},
  author={Merkle, Edgar C and Steyvers, Mark},
  journal={Decision Analysis},
  volume={10},
  number={4},
  pages={292--304},
  year={2013},
  publisher={INFORMS}
}

@article{bregman1967relaxation,
  title={The relaxation method of finding the common point of convex sets and its application to the solution of problems in convex programming},
  author={Bregman, Lev M},
  journal={USSR Computational Mathematics and Mathematical Physics},
  volume={7},
  number={3},
  pages={200--217},
  year={1967},
  publisher={Elsevier}
}

@article{banerjee2005clustering,
  title={Clustering with Bregman divergences},
  author={Banerjee, Arindam and Merugu, Srujana and Dhillon, Inderjit S and Ghosh, Joydeep},
  journal={Journal of machine learning research},
  volume={6},
  number={Oct},
  pages={1705--1749},
  year={2005}
}

@article{dawid2007geometry,
  title={The geometry of proper scoring rules},
  author={Dawid, A Philip},
  journal={Annals of the Institute of Statistical Mathematics},
  volume={59},
  number={1},
  pages={77--93},
  year={2007},
  publisher={Springer}
}

@article{saerens2002adjusting,
  title={Adjusting the outputs of a classifier to new a priori probabilities: a simple procedure},
  author={Saerens, Marco and Latinne, Patrice and Decaestecker, Christine},
  journal={Neural Comp.}, 
  volume={14},
  number={1},
  pages={21--41},
  year={2002},
  publisher={MIT Press}
}

@article{sugiyama2007covariate,
  title={Covariate shift adaptation by importance weighted cross validation},
  author={Sugiyama, Masashi and Krauledat, Matthias and M{\"u}ller, Klaus-Robert},
  journal={Journal of Machine Learning Research},
  volume={8},
  number={May},
  pages={985--1005},
  year={2007}
}

@inproceedings{kull2015novel,
  title={Novel decompositions of proper scoring rules for classification: Score adjustment as precursor to calibration},
  author={Kull, Meelis and Flach, Peter},
  booktitle={Joint European Conf. on Machine Learning and Knowledge Discovery in Databases},
  pages={68--85},
  year={2015},
  organization={Springer}
}

@article{japkowicz2002class,
  title={The class imbalance problem: A systematic study},
  author={Japkowicz, Nathalie and Stephen, Shaju},
  journal={Intelligent data analysis},
  volume={6},
  number={5},
  pages={429--449},
  year={2002},
  publisher={IOS Press}
}

@article{shimodaira2000improving,
  title={Improving predictive inference under covariate shift by weighting the log-likelihood function},
  author={Shimodaira, Hidetoshi},
  journal={J. of Stat. Planning and Inference},
  volume={90},
  number={2},
  pages={227--244},
  year={2000},
  publisher={Elsevier}
}

@article{gretton2009covariate,
  title={Covariate shift by kernel mean matching},
  author={Gretton, Arthur and Smola, Alexander J and Huang, Jiayuan and Schmittfull, Marcel and Borgwardt, Karsten M and Sch{\"o}lkopf, Bernhard},
  journal={Dataset shift in machine learning},
  pages={131--160},
  year={2009},
  publisher={MIT press}
}

@article{moreno2012unifying,
  title={A unifying view on dataset shift in classification},
  author={Moreno-Torres, Jose G and Raeder, Troy and Alaiz-Rodr{\'\i}guez, Roc{\'\i}o and Chawla, Nitesh V and Herrera, Francisco},
  journal={Pattern Recognition},
  volume={45},
  number={1},
  pages={521--530},
  year={2012},
  publisher={Elsevier}
}

@article{storkey2009training,
  title={When training and test sets are different: characterizing learning transfer},
  author={Storkey, Amos},
  journal={Dataset shift in machine learning},
  pages={3--28},
  year={2009},
  publisher={Citeseer}
}

@article{ditzler2015learning,
  title={Learning in nonstationary environments: A survey},
  author={Ditzler, Gregory and Roveri, Manuel and Alippi, Cesare and Polikar, Robi},
  journal={IEEE Computational Intelligence Magazine},
  volume={10},
  number={4},
  pages={12--25},
  year={2015},
  publisher={IEEE}
}

@inproceedings{kull2014patterns,
  title={Patterns of dataset shift},
  author={Kull, Meelis and Flach, Peter},
  booktitle={First International Workshop on Learning over Multiple Contexts (LMCE) at ECML-PKDD},
  year={2014}
}

@misc{heckman1977sample,
  title={Sample selection bias as a specification error (with an application to the estimation of labor supply functions)},
  author={Heckman, James J},
  year={1977},
  publisher={National Bureau of Economic Research Cambridge, Mass., USA}
}

@article{hein2009binary,
  title={Binary classification under sample selection bias},
  author={Hein, Matthias},
  journal={Dataset Shift in Machine Learning (J. Candela, M. Sugiyama, A. Schwaighofer and N. Lawrence, eds.). MIT Press, Cambridge, MA},
  pages={41--64},
  year={2009}
}

@article{puhani2000heckman,
  title={The Heckman correction for sample selection and its critique},
  author={Puhani, Patrick},
  journal={Journal of economic surveys},
  volume={14},
  number={1},
  pages={53--68},
  year={2000},
  publisher={Wiley Online Library}
}

@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge Univ. Press}
}

@article{OpenML2013,
author = {Vanschoren, Joaquin and van Rijn, Jan N. and Bischl, Bernd and Torgo, Luis},
title = {{OpenML}: Networked Science in Machine Learning},
journal = {SIGKDD Explorations},
volume = {15},
number = {2},
year = {2013},
pages = {49--60},
publisher = {ACM},
address = {New York, NY, USA},
}

@article{OpenMLR2017,
author = {Casalicchio, Giuseppe and Bossek, Jakob and Lang, Michel and Kirchhoff, Dominik and Kerschke, Pascal and Hofner, Benjamin and Seibold, Heidi and Vanschoren, Joaquin and Bischl,Bernd},
title = {OpenML: An R package to connect to the machine learning platform OpenML},
journal = {Computational Statistics},
volume = {32},
number = {3},
year = {2017},
pages = {1--15},
url = {http://doi.acm.org/10.1007/s00180-017-0742-2},
doi = {10.1007/s00180-017-0742-2},
publisher = {Springer Nature}
}

@inproceedings{zadrozny2001learning,
  title={Learning and making decisions when costs and probabilities are both unknown},
  author={Zadrozny, Bianca and Elkan, Charles},
  booktitle={Proceedings of the seventh ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={204--213},
  year={2001},
  organization={ACM}
}

@article{degroot1983comparison,
  title={The comparison and evaluation of forecasters},
  author={DeGroot, Morris H and Fienberg, Stephen E},
  journal={The statistician},
  pages={12--22},
  year={1983},
  publisher={JSTOR}
}

@Manual{R2015,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2015},
    url = {https://www.R-project.org/},
  }
  
@Manual{RStudio2016,
    title = {RStudio: Integrated Development Environment for R},
    author = {{RStudio Team}},
    organization = {RStudio, Inc.},
    address = {Boston, MA},
    year = {2016},
    url = {http://www.rstudio.com/},
}

@article{cvxpy,
  author  = {Steven Diamond and Stephen Boyd},
  title   = {{CVXPY}: A {P}ython-Embedded Modeling Language for Convex Optimization},
  journal = {Journal of Machine Learning Research},
  year    = {2016},
  volume  = {17},
  number  = {83},
  pages   = {1--5},
}

@inproceedings{stellato2018osqp,
  title={OSQP: An operator splitting solver for quadratic programs},
  author={Stellato, Bartolomeo and Banjac, Goran and Goulart, Paul and Bemporad, Alberto and Boyd, Stephen},
  booktitle={2018 UKACC 12th International Conference on Control (CONTROL)},
  pages={339--339},
  year={2018},
  organization={IEEE}
}

@inproceedings{domahidi2013ecos,
  title={ECOS: An SOCP solver for embedded systems},
  author={Domahidi, Alexander and Chu, Eric and Boyd, Stephen},
  booktitle={2013 European Control Conference (ECC)},
  pages={3071--3076},
  year={2013},
  organization={IEEE}
}

@misc{o2016scs,
  title={SCS: Splitting conic solver, version 1.2. 6},
  author={O’Donoghue, Brendan and Chu, Eric and Parikh, Neal and Boyd, S},
  year={2016}
}

@incollection{bauschke2001joint,
  title={Joint and separate convexity of the {Bregman} distance},
  author={Bauschke, Heinz H and Borwein, Jonathan M},
  booktitle={Studies in Computational Mathematics},
  volume={8},
  pages={23--36},
  year={2001},
  publisher={Elsevier}
}

@article{pan2010survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2010},
  publisher={IEEE}
}

@article{weiss2016survey,
  title={A survey of transfer learning},
  author={Weiss, Karl and Khoshgoftaar, Taghi M and Wang, DingDing},
  journal={Journal of Big Data},
  volume={3},
  number={1},
  pages={9},
  year={2016},
  publisher={SpringerOpen}
}
